Visual Story Post-Editing

We introduce the first dataset for human edits of machine-generated visual stories and explore how these collected edits may be used for the visual story post-editing task. The dataset, VIST-Edit, includes 14,905 human edited versions of 2,981 machine-generated visual stories. The stories were generated by two state-of-the-art visual storytelling models, each aligned to 5 human-edited versions. We establish baselines for the task, showing how a relatively small set of human edits can be leveraged to boost the performance of large visual storytelling models. We also discuss the weak correlation between automatic evaluation scores and human ratings, motivating the need for new automatic metrics.

==> ACL_2019_0604(LaTex)/abstract.tex <==


We introduce the first dataset for \textbf{human edits of machine-generated visual stories} and explore how these collected edits may be used for the \textit{visual story post-editing} task.
The dataset, \dataset\footnote{\dataset: https://github.com/tingyaohsu/VIST-Edit}, includes 14,905 human-edited versions of 2,981 machine-generated visual stories. The stories were generated by two state-of-the-art visual storytelling models, each aligned to 5 human-edited versions.
We establish baselines for the task, showing how a relatively small set of human edits can be leveraged to boost the performance of large visual storytelling models.
We also discuss the weak correlation between automatic evaluation scores and human ratings, motivating the need for new automatic metrics.


%-------------- end of document -------------

\begin{comment}

%%%%%%%%%%%%%%%%%%%%before edited by yen-chia
We introduce the first dataset for \textbf{human edits of machine-generated visual stories} and explore how these collected edits may be used for the task of \textit{visual story post-editing.}
The first release of this dataset, \dataset\footnote{\dataset will be available upon publication.}, includes 14,905 human-edited versions of 2,981 machine-generated visual stories \textcolor{red}{merge with previous sentence?}. The stories were generated by two state-of-the-art visual storytelling models, each aligned to 5 human-edited versions.
We establish several baselines for the visual story automatic post-editing task, showing how a relatively small set of human edits can be leveraged to boost the performance of visual storytelling models.
We also discuss \textcolor{red}{stress} the weak correlation between automatic evaluation scores and human ratings, motivating the need for new automatic metrics.
%%%%%%%%%%%%%%%%%%%%


We introduce the first dataset for \textbf{human edits on machine-generated visual stories}, and explore how these collected edits may be used for the task of \textit{visual story post-editing.}
The first release of this dataset, \dataset v1\footnote{\dataset will be available upon publication.}, includes 2,981 machine-generated visual stories and 14,905 human-edited versions of them.
The stories were generated by two state-of-the-art visual storytelling models, and each aligned to 5 human-edited versions.
We establish several baselines for the visual story automatic post-editing task, showing how a relatively small set of human edits can be leveraged to boost the performance of visual storytelling models.
We also discuss the weak correlation between METEOR scores and human ratings, motivating the needs of new automatic evaluation metrics.

%81,743 unique photos in 20,211 sequences, aligned to both descriptive (caption) and story language. 

 We establish several
strong baselines for the storytelling task, and
motivate an automatic metric to benchmark
progress. Modelling concrete description as
well as figurative and social language, as provided in this dataset and the storytelling task,
has the potential to move artificial intelligence
from basic understandings of typical visual
scenes towards more and more human-like understanding of grounded event structure and
subjective expression.



%The first release of this dataset, SIND1 v.1,
includes 81,743 unique photos in 20,211 sequences, aligned to both descriptive (caption)
and story language


A large body of work has been devoted to automatically generating short stories from image sequences. However, literature has little to say about how users can \textit{use} these generated stories in their day-to-day lives, {\em e.g.,} sharing stories about their holiday photos on social media. Given the lower quality of text generated by visual storytelling models, users will nearly inevitably need to edit these text before putting them to real use. In this paper, we introduce \textit{visual story post-editing}. We argue that user's post-editing is a highly likely step when automatic visual storytelling models are brought out of the lab and deployed to actual users. The systematic differences between an original automatic story and its user-edited version can be learned by a neural-based post-editing model from pre- and post-edited story pairs generated by users. At run time, we can then apply this post-editing model on stories generated from image sequences to improve the resulting story quality. Our experiments on 4,810 pre- and post-edited story pairs show that our proposed model reduces repetition in texts, adds more details to narratives, makes the stories more human-like; and most importantly, users become more willing to share the edited visual stories.

\end{comment}


==> ACL_2019_0604(LaTex)/auto-edit-as-ai-task.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\scriptsize	
\addtolength{\tabcolsep}{-0.03cm} 
\begin{tabular}{|l|rrrrrr|rrrrrr|}
\hline
\multicolumn{1}{|c|}{\textit{}} & \multicolumn{6}{c|}{\textit{\textbf{AREL}}} & \multicolumn{6}{c|}{\textit{\textbf{GLAC}}} \\ \hline
Edited By & Focus & Coherence & Share & Human & Grounded & Detailed & Focus & Coherence & Share & Human & Grounded & Detailed \\ \hline
\textbf{N/A} & 3.487 & 3.751 & 3.763 & 3.746 & 3.602 & 3.761 & 3.878 & 3.908 & 3.930 & 3.817 & 3.864 & 3.938 \\ \hline
\textbf{TF (T)} & 3.433 & 3.705 & 3.641 & 3.656 & 3.619 & 3.631 & 3.717 & 3.773 & 3.863 & 3.672 & 3.765 & 3.795 \\
\textbf{TF (T+I)} & \textbf{3.542} & 3.693 & 3.676 & 3.643 & 3.548 & 3.672 & 3.734 & 3.759 & 3.786 & 3.622 & 3.758 & 3.744 \\
\textbf{LSTM (T)} & \textbf{3.551} & \textbf{3.800} & \textbf{3.771} & \textbf{3.751} & \textbf{3.631} & \textbf{3.810} & \textbf{3.894} & 3.896 & 3.864 & \textbf{3.848} & 3.751 & 3.897 \\
\textbf{LSTM (T+I)} & \textbf{3.497} & 3.734 & 3.746 & 3.742 & 3.573 & 3.755 & 3.815 & 3.872 & 3.847 & 3.813 & 3.750 & 3.869 \\ \hline
\textbf{Human} & 3.592 & 3.870 & 3.856 & 3.885 & 3.779 & 3.878 & 4.003 & 4.057 & 4.072 & 3.976 & 3.994 & 4.068 \\ \hline
\end{tabular}
\addtolength{\tabcolsep}{0.03cm} 
%\vspace{-.5pc}
\caption{Human evaluation results. Five human judges on MTurk rate each story on the following six aspects, using a 5-point Likert scale (from Strongly Disagree to Strongly Agree):
Focus,
Structure and Coherence, 
Willing-to-Share (``I Would Share''),
Written-by-a-Human (``This story sounds like it was written by a human.''),
Visually-Grounded, and
Detailed. We take the average of the five judgments as the final score for each story.
LSTM(T) improves all aspects for stories by AREL, and improves ``Focus'' and ``Human-like'' aspects for stories by GLAC.
%These results demonstrate that a relatively small set of human edits can be used to boost the story quality of an existing VIST model.
}
\label{tab:human-eval}
%\vspace{-1pc}
\end{table*}

We report baseline experiments on the visual story post-editing task in Table~\ref{tab:human-eval}.
AREL's post-editing models are trained on the augmented AREL training set and evaluated on the AREL test set of \dataset, and GLAC's models are tested using GLAC sets, too.
Figure~\ref{fig:representative-story} shows examples of the output.
Human evaluations (Table~\ref{tab:human-eval}) indicate that the post-editing model improves visual story quality.

\subsection{Methods}

Two neural approaches, Long short-term memory (LSTM) and Transformer, are used as baselines, where we experiment using {\em (i)} text only (T) and {\em (ii)} both text and images (T+I) as inputs.

\paragraph{LSTM}
An LSTM seq2seq model is used~\cite{sutskever2014sequence}.
For the text-only setting, the original stories and the human-edited stories are treated as source-target pairs.
For the text-image setting, we first extract the image features using the pre-trained ResNet-152 model~\cite{he2016deep} and represent each image as a 2048-dimensional vector. 
We then apply a dense layer on image features in order to both fit its dimension to the word embedding and learn the adjusting transformation. 
By placing the image features in front of the sequence of text embedding, the input sequence becomes a matrix $\in \mathbb{R}^{(5+len) \times dim}$, where $len$ is the text sequence length, $5$ means 5 photos, and $dim$ is the dimension of the word embedding.
The input sequence with both image information and text information is then encoded by LSTM, identical as in the text-only setting.

\paragraph{Transformer (TF)}
%\kenneth{TODO CY: proofread this part}
We also use the Transformer architecture~\cite{vaswani2017attention} as baseline.
The text-only setup and image feature extraction are identical to that of LSTM.
For Transformer, the image features are attached at the end of the sequence of text embedding to form an image-enriched embedding.
It is noteworthy that the position encoding is only applied on text embedding.
%We add position encoding only on the text embedding part. %except the image features. 
The input matrix $\in \mathbb{R}^{(len+5) \times dim}$ is then passed into the Transformer as in the text-only setting.
%\kenneth{why we didn't cite the Transformer paper?}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{fig/representative_example_stories_full_width.png}
    \caption{Example stories generated by baselines.}
    %\vspace{-2pc}
    \label{fig:representative-story}
    %\vspace{1pc}
\end{figure*}

\subsection{Experimental Setup and Evaluation}

\begin{comment}



% \ding{172}
% reference: https://tex.stackexchange.com/questions/199026/how-can-i-draw-circled-integers-with-the-same-size-by-tikz
\begin{table}[]
\centering
\scriptsize
%\footnotesize
\addtolength{\tabcolsep}{-0.1cm} 
\begin{tabular}{llrrrr}

\toprule \hline
  & \textbf{Data Includes}  & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts}\\ \hline
\ding{172} & AREL       & .110   & .099  & .063  & .062           \\
\ding{173} &  LSTM-Edited AREL & .106   & .109  & .067 & .205         \\
\ding{174} & \ding{172}+\ding{173}                     & .095   & .092  & .059    & .116              \\ \hline
\ding{175} & GLAC   & .222   & .203  & .140    &  .151             \\
\ding{176} &  LSTM-Edited GLAC                & .163   & .176  & .138    &    .087           \\
\ding{177} & \ding{175}+\ding{176}                     & .196   & .194  & .148    & .116              \\ \hline
\ding{178} & \ding{172}+\ding{175}                     & .091   & .086  & .059    & .088              \\
\ding{179} & \ding{173}+\ding{176}                     & .089   & .103  & .067    & .101              \\
\ding{180} & \ding{172}+\ding{173}+\ding{175}+\ding{176} & .090   & .096  & .069 & .094             \\ \hline \bottomrule
\end{tabular}
\addtolength{\tabcolsep}{0.1cm} 
\caption{Spearman rank-order correlation $\rho$ between the automatic evaluation scores (sum of all six aspects) and human judgment calculated using different data combination. GLAC(N=202), AREL(N=97)\hsu{modify after 2(Spearman)}}
\label{tab:auto-human-cor}
\end{table}

\end{comment}

\paragraph{Data Augmentation}
%In the normal setting, we construct five training samples by paring the original story with the human-edited one but this leads to a limited amount of data. 
%In order to augment the data, 
In order to obtain sufficient training samples for neural models, we pair \textit{less}-edited stories with \textit{more}-edited stories of the same photo sequence to augment the data.
%Taking advantage of the fact that we have 
In \dataset, five human-edited stories are collected for each photo sequence.
We use the human-edited stories that are less edited -- measured by its Normalized Damerau-Levenshtein distance \cite{levenshtein1966binary,damerau1964technique} to the original story -- as the source and pair them with the stories that are more edited (as the target.)
%Normalized Damerau-Levenshtein distance \cite{levenshtein1966binary,damerau1964technique} is used to measure the similarity between two stories.
%That is to say, we pair a less-edited story with a more-edited story for data augmentation.
This data augmentation strategy gives us in total fifteen ($\left ( ^5_2 \right )+5=15$) training samples given five human-edited stories.%\kenneth{this can be more clear}


\paragraph{Human Evaluation}
Following the evaluation procedure of the first VIST Challenge~\cite{mitchell2018proceedings}, for each visual story, we recruit five human judges on MTurk to rate it on six aspects (at \$0.1/HIT.)
We take the average of the five judgments as the final scores for the story.
%\kenneth{saying it's average}
%Workers are asked to rate on the following six aspects, using a 5-point Likert scale (from Strongly Disagree to Strongly Agree): 
%Focus, 
%Coherence,
%Willing-to-Share,
%Written-by-a-Human,
%Visually-Grounded, and 
%Detailed.
Table~\ref{tab:human-eval} shows the results.
The LSTM using text-only input outperforms all other baselines.
It improves all six aspects for stories by AREL, and improves ``Focus'' and ``Human-like'' aspects for stories by GLAC.
These results demonstrate that a relatively small set of human edits can be used to boost the story quality of an existing large VIST model.
Table~\ref{tab:human-eval} also suggests that the quality of a post-edited story is heavily decided by its pre-edited version.
Even after editing by human editors, AREL's stories still do not achieve the quality of pre-edited stories by GLAC.
%
The inefficacy of image features and Transformer model might be caused by the small size of \dataset.
It also requires further research to develop a post-editing model in a multimodal context.

%good pre-edited stories result in good post-edited stories


%Although Transformer has achieved great successes on many NLP tasks, its heavy structure with fully-connected attention connections leads to dependencies on large training data








%======================= end of document ====================

\begin{comment}

\footnote{Given 5 human-edited stories, we could generate $4$ samples by paring the story with the lowest distance to the other four stories, $3$ samples from the second lowest one to the other three stories, and so on. Eventually we could have $4+3+2+1=10$ stories.} 

%between the human-edited stories and the machine-generated story. 
%The edit distance indicates the degree of human editing where $1.0$ means the edited story and the original story have nothing in common and $0.0$ means they are totally identical.
%We then generate training samples by pairing a human-edited story with lower edit distance to another human-edited story with higher edit distance.

The system overcame the problem of limited APE training data by generating a large amount of artificial training data with back-translation~\cite{sennrich2015improving}.
The idea was to use two phase-based MT systems to translate German to English and then back to German.
The original German, the translated English, and the back-translated German are treated as the post-edited, source, and the machine-translated sentences respectively.


For the text-only setting, the source-target pairs is identical as that of LSTM.
For the text-image setting, we again use the image features extracted from the last convolutional layer of pre-trained ResNet-152 mdoel \cite{he2016deep} and apply a dense layer to adjust the dimension and learn the transformation. 


%% LSTM method
We use the LSTM seq2seq model \cite{sutskever2014sequence} as the main structure. 
For text-only setting, the original stories and the human edited stories are treated as the source-target pairs in the translation problem. 
To incorporate the image information, we first extract the image features by the pretrained ResNet-152 model \cite{he2016deep} where each image is represented as a 2048-dimension vector. 
%We put all the image feature in an embedding layer so the photo sequence could work like the process of handling a text sequence. 
%A photo sequence which is consist of five photos is then represented by a matrix $\textbf{P}  \in \mathbb{R}^{5 \times 2048}$. 
We apply a dense layer on image features in order to both fit its dimension to the word embedding and learn the adjusting transformation. 
%After passing through the dense layer, we get another matrix $\textbf{P}'  \in \mathbb{R}^{5 \times dim}$ where $dim$ is the dimension of the word embedding. 
By placing the image features in front of the word embeddings, the source sequence becomes a matrix $\in \mathbb{R}^{(len+5) \times dim}$ where $len$ is the text sequence length, $5$ means 5 photos, and $dim$ stands for the dimension of the word embedding. We feed $\textbf{M}$ into the LSTM seq2seq model as what we did in the text-only setting.
%We then concatenate $\textbf{P}'$ and the text information matrix together to get $\textbf{M} \in \mathbb{R}^{(len+5) \times dim}$ where $len$ is the text sequence length. 

%% Transformer
We use a classical Machine Translation model - Transformer \cite{vaswani2017attention} as our main structure. 
For the text part, we use auto-generated story and human-edit story as our source-target pairs for the input.
For the image plus text part, we first extract the image features from the last convolutional layer of pre-trained ResNet-152 mdoel which is a 2048-dimension vector.
Then we pass all the image feature through an embedding layer to make them fit the same dimension as text sequence. 
One photo sequence contains five photos, which is a matrix $\textbf{T} \in 5 \times 2048 $. 
After passing through the embedded layer, we obtain the output matrix $\textbf{T}' \in 5 \times dim $, which is the same dimension of word embedding. 
We simply concatenate $\textbf{T}$ and $\textbf{T}'$, which represent the matrix of word embedding of text sequence. 
We treat each image feature as one word vector and get the new matrix $\textbf{S} \in (5 + $length$) \times dim$, where $length$ means the length of text sequence.
Finally, we put $\textbf{S}$ into our Transformer model to generate the sentence.

\begin{table*}[t]
%\scriptsize	
\small
\begin{tabular}{@{}lrrrrrr|rrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textit{}} & \multicolumn{6}{c|}{\textit{\textbf{AREL}}} & \multicolumn{6}{c}{\textit{\textbf{GLAC}}} \\ \midrule
Edited By & Focused & Coherent & Share & Human & Grounded & Detailed & Focused & Coherent & Share & Human & Grounded & Detailed \\ \midrule
\textbf{N/A} & 3.487 & 3.751 & 3.763 & 3.746 & 3.602 & 3.761 & 3.878 & 3.908 & 3.930 & 3.817 & 3.864 & 3.938 \\ \midrule
\textbf{TF (T)} & 3.433 & 3.705 & 3.641 & 3.656 & 3.619 & 3.631 & 3.717 & 3.773 & 3.863 & 3.672 & 3.765 & 3.795 \\
\textbf{TF (T+I)} & \textbf{3.542} & 3.693 & 3.676 & 3.643 & 3.548 & 3.672 & 3.734 & 3.759 & 3.786 & 3.622 & 3.758 & 3.744 \\
\textbf{LSTM (T)} & \textbf{3.551} & \textbf{3.800} & \textbf{3.771} & \textbf{3.751} & \textbf{3.631} & \textbf{3.810} & \textbf{3.894} & 3.896 & 3.864 & \textbf{3.848} & 3.751 & 3.897 \\
\textbf{LSTM (T+I)} & \textbf{3.497} & 3.734 & 3.746 & 3.742 & 3.573 & 3.755 & 3.815 & 3.872 & 3.847 & 3.813 & 3.750 & 3.869 \\ \midrule
\textbf{Human} & 3.592 & 3.870 & 3.856 & 3.885 & 3.779 & 3.878 & 4.003 & 4.057 & 4.072 & 3.976 & 3.994 & 4.068 \\ \bottomrule
\end{tabular}
 \caption{Human evaluation results for visual story post-editing models.}
\end{table*}
\end{comment}



%\paragraph{Automatic Evaluation}

%\paragraph{Human Judgment}


==> ACL_2019_0604(LaTex)/conclusion.tex <==
\dataset, the first dataset for \textbf{human edits of machine-generated visual stories}, is introduced.
We argue that human editing on machine-generated stories is unavoidable, and such edited data can be leveraged to enable automatic post-editing.
We have established baselines for the task of visual story post-editing, and have motivated the need for a new automatic evaluation metric.


%-------------- end of document -------------

\begin{comment}




METEOR as an automatic metric to evaluate
progress on this task moving forward.


edit stories generated by machines


We have established 

The automatic post-editing task, on the other hand, revises the story generated from visual storytelling models, given both a machine-generated story and a photo sequence. It treats the VIST system as a black box that is fixed and not modifiable. 

The goal of automatic visual story post-editing is to 

correct systematic errors of the VIST system and leverage the inevitable user edit data to improve story quality. 




We
argue that modelling the more figurative and social language captured in this dataset is essential for
evolving AI towards more human-like understanding. 

We have established several baselines for the task of visual story post-editing, and have motivated METEOR as an automatic metric to evaluate
progress on this task moving forward.





Conclusion:
1. The more users edit, the worse the story quality is.
2. Existing auto eval metrics doesn't help much.
3. Post-edits, as an AI task, is do-able!

Future Work:
1. Gain a deeper understanding about user's perception of generated stories
2. 
3. 

\end{comment}

==> ACL_2019_0604(LaTex)/data.tex <==
\paragraph{Obtaining Machine-Generated Visual Stories} 
%Many prior works have been proposed for the visual storytelling task.
%In this paper, 
This \dataset dataset contains visual stories generated by two state-of-the-art models, \textbf{GLAC} and \textbf{AREL}.
GLAC (Global-Local Attention Cascading Networks)~\cite{kim2018glac} achieved the highest human evaluation score in the first VIST Challenge~\cite{mitchell2018proceedings}.
We obtain the pre-trained GLAC model provided by the authors via Github and run it on the entire VIST test set and obtain 2,019 stories.
%\kenneth{Did we retrain GLAC? How did we get the model?}\hsu{We use the pretrained model provided from the authors on Github, link: https://github.com/tkim-snu/GLACNet}
AREL (Adversarial REward Learning)~\cite{acl2018wang} was the earliest available implementation online, and achieved the highest METEOR score on public test set in the VIST Challenge.
We also acquire a small set of human edits for 962 AREL's stories generated using VIST test set, collected by Hsu {\em et al.}~\shortcite{hsu2019users}.

%We ran GLAC on the VIST test set and obtained 2,019 stories; and we acquired AREL's stories from Hsu {\em et al.}'s study~\cite{hsu2019users}, in which 962 stories were generated using the VIST test set.

\paragraph{Crowdsourcing Edits}
For each machine-generated visual story, we recruit five crowd workers from Amazon Mechanical Turk (MTurk) to revise it (at \$0.12/HIT,) respectively.
We instruct workers to edit the story ``as if these were your photos, and you would like using this story to share your experience with your friends.''
We also ask workers to stick with the photos of the original story so that workers would not ignore the machine-generated story and write a new one from scratch.
Figure~\ref{fig:ui} shows the interface.
For GLAC, we collect 2,019 $\times$ 5 = 10,095 edited stories in total; and for AREL, 962 $\times$ 5 = 4,810 edited stories have been collected by Hsu {\em et al.}~\shortcite{hsu2019users}.


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/interface.png}
    %\vspace{-1.5pc}
    \caption{Interface for visual story post-editing. An instruction (not shown to save space) is given and workers are asked to stick with the plot of the original story.}
    \label{fig:ui}
    %\vspace{-1.3pc}
\end{figure}

\paragraph{Data Post-processing}
We tokenize all stories using CoreNLP~\cite{coreNLP} and replace all people names with generic [male/female] tokens.
Each of GLAC and AREL set is released as training, validation, and test following an 80\%, 10\%, 10\% split, respectively.



\subsection{What do people edit?}
We analyze human edits for GLAC and AREL.
First, crowd workers systematically \textbf{increase lexical diversity}.
We use type-token ratio (TTR), the ratio between the number of word types and the number of tokens, to estimate the lexical diversity of a story~\cite{1af8cfb45ecf4823b5e14c69b80d4d5a}.
Figure~\ref{fig:ttr} shows significant (p\textless.001, paired t-test) positive shifts of TTR for both AREL and GLAC, which confirms the findings in Hsu {\em et al.}~\shortcite{hsu2019users}.
Figure~\ref{fig:ttr} also indicates that GLAC generates stories with higher lexical diversity than that of AREL.



\begin{figure}[thbp]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/ttr_shift.png}
    %\vspace{-1.5pc}
    \caption{KDE plot of type-token ratio (TTR) for pre-/post-edited stories. People increase lexical diversity in machine-generated stories for both AREL and GLAC.}
    \label{fig:ttr}
    %\vspace{-1pc}
\end{figure}



Second, people \textbf{shorten AREL's stories but lengthen GLAC's stories.}
We calculate the average number of Part-Of-Speech (POS) tags for tokens in each story using the python NLTK~\cite{bird2009natural} package, as shown in Table~\ref{tab:pos-stats}.
%\kenneth{TODO Edward: update the following numbers to match with the table.}
We also find that the average number of tokens in an AREL story (43.0, SD=5.0) decreases (41.9, SD=5.6) after human editing, while 
that of GLAC (35.0, SD=4.5) increases (36.7, SD=5.9).
Hsu has observed that people often replace ``determiner/article + noun'' phrases ({\em e.g.,} ``a boy'') with pronouns ({\em e.g.,} ``he'') in AREL stories~\shortcite{hsu2019users}.
However, this observation cannot explain the story lengthening in GLAC, where each story on average has an increased 0.9 nouns after editing.
Given the average per-story edit distances~\cite{levenshtein1966binary,damerau1964technique} for AREL (16.84, SD=5.64) and GLAC (17.99, SD=5.56) are similar, this difference is unlikely to be caused by deviation in editing amount.


\begin{table}[h]
    \scriptsize
    \centering
    \addtolength{\tabcolsep}{-0.165cm}
    \begin{tabular}{lrrrrrrrrrrr}
        \toprule
        \resizebox{0.55cm}{!}{\textbf{AREL}}     &    \textbf{.} & \textbf{ADJ} &  \textbf{ADP} &  \textbf{ADV} & \textbf{CONJ} &  \textbf{DET} & \textbf{NOUN} & \textbf{PRON} & \textbf{PRT} & \textbf{VERB} & \textbf{Total} \\ \hline
        \textbf{Pre}      &  5.2 & 3.1 &  3.5 &  1.9 &  0.5 &  8.1 & 10.1 &  2.1 & 1.6 &  6.9 & 43.0 \\
        \textbf{Post}     &  4.7 & 3.1 &  3.4 &  1.9 &  0.8 &  7.1 &  9.9 &  2.3 & 1.6 &  7.0 & 41.9 \\
        \textbf{$\Delta$} & -0.5 & 0.0 & -0.1 & -0.1 &  0.4 & -1.0 & -0.2 &  0.2 & 0.0 &  0.1 & -1.2 \\ 
        \bottomrule
        % \multicolumn{13}{!}{\vspace{-1cm} } \\
        \toprule
        \resizebox{0.55cm}{!}{\textbf{GLAC}}     &    \textbf{.} & \textbf{ADJ} &  \textbf{ADP} &  \textbf{ADV} & \textbf{CONJ} &  \textbf{DET} & \textbf{NOUN} & \textbf{PRON} & \textbf{PRT} & \textbf{VERB} & \textbf{Total} \\ \hline
        \textbf{Pre}      &  5.0 &  3.3 & 1.7 &  1.9 &  0.2 &  6.5 &  7.4 &  1.2 & 0.8 &  6.9 & 35.0 \\
        \textbf{Post}     &  4.5 &  3.2 & 2.4 &  1.8 &  0.8 &  6.1 &  8.3 &  1.5 & 1.0 &  7.0 & 36.7 \\ 
        \textbf{$\Delta$} & -0.5 & -0.1 & 0.7 & -0.1 &  0.6 & -0.3 &  0.9 &  0.3 & 0.2 &  0.1 &  1.7 \\ 
        \bottomrule
    \end{tabular}
    \addtolength{\tabcolsep}{0.165cm}
    %\vspace{-.5pc}
    \caption{Average number of tokens with each POS tag per story. ($\Delta$: the differences between post- and pre-edit stories. NUM is omitted because it is nearly 0. Numbers are rounded to one decimal place.)}\label{tab:pos-stats}
    %\vspace{-1pc}
\end{table}

\textit{Deleting} extra words requires much less time than other editing operations~\cite{popovic2014relations}.
Per Figure~\ref{fig:ttr}, AREL's stories are much more repetitive.
We further analyze the type-token ratio for nouns (${TTR}_{noun}$) and find AREL generates duplicate nouns.
The average ${TTR}_{noun}$ of an AREL's story is 0.76 while that of GLAC is 0.90.
For reference, the average ${TTR}_{noun}$ of a human-written story (the entire VIST dataset) is 0.86.
Thus, we hypothesize workers prioritized their efforts in deleting repetitive words for AREL, resulting in the reduction of story length.





%==================== end of doc ================================

\begin{comment}






\begin{figure}[bhp]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/noun_example.pdf}
    \caption{Example}
    %\label{fig:ttr}
\end{figure}



people usually shorten AREL's stories 



We suspect that 



post-edited stories 

observe a systematic increase of type-token ratio (TTR) in post-edited stories. 




TTR, calculated as the ratio between the number of words types and the number of tokens, is a common indicator of lexical diversity of a document~\cite{1af8cfb45ecf4823b5e14c69b80d4d5a}.

as shown in Figure~\ref{fig:ttr}.






First, people \textbf{shorten AREL's stories but lengthen GLAC's stories.}
As shown in Table~\ref{tab:pos-stats}, the post-edited visual stories from GLAC are significantly longer ($p < 0.001$).
%
Second, people \textbf{increase lexical diversity}.
We observe a systematic increase of type-token ratio (TTR) for models, as shown in Figure~\ref{fig:ttr}.
TTR, calculated as the ratio between the number of words types and the number of tokens, is often used to estimate lexical diversity of a document.


index of lexical diversity [5], which is calculated as the ratio between the number
of different words (types) Ntype and the total number of words (tokens) Ntoken of a text unit, i.e.,
TTR = Ntype /Ntoken. A higher TTR indicates a higher lexical diversity. Per our analysis, the average
TTR for an automatic story is 0.62 (SD = 0.09), while the average TTR for an edited story is 0.72 (SD
= 0.06). This difference is statistically significant (paired t-test, $p < 0.001$, N = 4810). This result
suggested that users reduced the word redundancy and increased the lexical diversity in machinegenerated
stories. The normalized frequency histogram of TTR of pre- and post-edited stories are
shown in Figure 4.



Finally, 

Edited stories are slightly shorter







Hsu {\em et al.} has collected a small set of human edits for 962 AREL's stories generated using VIST test set~\shortcite{hsu2019users}.
We acquired their data in \dataset.





the NLTK toolkit~\cite{bird2009natural}

\paragraph{Move to ``ideal'' story length.}



\paragraph{Increase lexical diversity.}
We echoed~\cite{hsu2019users}

\paragraph{People put a fix amount of effort in editing.}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/ab_ed_dist_avg.png}
    \caption{KDE plot of absolute edit distance between pre-/post-edited stories. People edit the same amount of operation for both AREL and GLAC.}
    \label{fig:ab_edit_distribution}
\end{figure}


%add TTR for NOUN here



We compute the edit distance \cite{levenshtein1966binary,damerau1964technique} between pre-/post-edited stories.
Since there are five post-edited stories for a given pre-edit story, we compute the average as edit distance.
%In order to compare whether people put the same amount of effort into different stories.
We only consider samples that appear in both AREL and GLAC. 
The average edit distance is 16.84 (SD=5.64) for AREL and 17.99 (SD=5.56) for GLAC. 
%We also plot the distribution of the edit distance in Figure~\ref{fig:ab_edit_distribution}. 
The high degree of similarity between two distributions (Figure~\ref{fig:ab_edit_distribution}) suggests that regardless of the story quality, people always do the same amount of editing operation.
% $0.12 -> a fix amount of editing



MTurk is a pay-per-task marketplace so workers tend to provide a similar amount of time an effort for a fixed given price, 



turn to realize MTurk is a pay-per-task marketplace so workers tend to provide a fixed amount of time an effort for a fixed given price, in our case, \$0.12/HIT.




requesters should expect a fixed amount of work for each task.


Hsu {\em et al.} observed that after human post-editing, an AREL story usually becomes shorter ($p<0.001$); however, we find the opposite for GLAC.




We analyzed the parts of speech of the words in each story.
The universal part-of-speech tagset\footnote{A Universal Part-of-Speech Tagset:\\ https://www.nltk.org/book/ch05.html} provided by NLTK toolkit was used.
The average number of tokens of each POS in a story is shown in Table~\ref{tab:pos-stats}.
We observed that the ``DET'' (determiner, article) tag contributes the most to the reduction of story length, while the number of ``PRON'' (pronoun) tags increased the most.
In order to understand the possible reasons behind this phenomenon, we observed the stories that had fewer DET tags but more PRON tags after post editing.
We found that the nouns with determiners and articles (DET) are often replaced by pronouns (PRON).
The following is a typical example, where the replacement texts are highlighted in red.









One explanation that could govern all these phenomena 

% \begin{table}[]
% \scriptsize
% \centering
% % \adjustbox{max width=\columnwidth}{
% \begin{tabular}{x{0.1cm}R{0.4cm}R{0.4cm}R{0.4cm}R{0.4cm}R{0.4cm}R{0.39cm}R{0.5cm}R{0.4cm}R{0.4cm}R{0.4cm}R{0.5cm}}
% \toprule
%           & .    & ADJ & ADP  & ADV & CONJ & DET  & NOUN & PRON & PRT & VERB & Total \\ \hline
% Pre  & 5.2  & 3.1 & 3.5  & 1.9 & 0.5  & 8.1  & 10.1 & 2.1  & 1.6 & 7.0  & 43.1  \\
% Post & 4.7  & 3.1 & 3.4  & 1.9 & 0.9  & 7.2  & 9.9  & 2.3  & 1.6 & 7.0  & 42.0  \\ \hline
% $\Delta$  & -0.5 & 0.0 & -0.1 & 0.0 & 0.4  & -0.9 & -0.2 & 0.2  & 0.0 & 0.0  & -1.1  \\ \bottomrule
% \end{tabular}
% % }
% \end{table}


% \begin{table*}[]
% \small
% \centering
% \begin{tabular}{x{0.5cm}R{0.3cm}rrrrrrrrrr}
% \toprule
%           & .    & ADJ  & ADP & ADV  & CONJ & DET  & NOUN & PRON & PRT & VERB & Total \\ \hline
% Pre  & 5.0  & 3.4  & 1.7 & 1.9  & 0.3  & 6.5  & 7.4  & 1.2  & 0.8 & 6.9  & 35.1  \\
% Post & 4.5  & 3.2  & 2.4 & 1.8  & 0.8  & 6.1  & 8.3  & 1.5  & 1.0 & 7.0  & 36.6  \\ \hline
% $\Delta$  & -0.5 & -0.2 & 0.7 & -0.1 & 0.5  & -0.4 & 0.9  & 0.3  & 0.2 & 0.1  & 1.5   \\ \bottomrule
% \end{tabular}
% \end{table*}

% \paragraph{POS???}
% \begin{table}
% %\begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{fig/both_pos_fig.pdf}
%     \caption{POS\kenneth{why i'm looking at this? What can I learn from it?}}
%     \label{tab:pos-stats}
% %\end{figure}

% \end{table}

\end{comment}




==> ACL_2019_0604(LaTex)/discussion.tex <==
\paragraph{Automatic evaluation scores do not reflect the quality improvements.}
APE for MT has been using automatic metrics, such as BLEU, to benchmark progress~\cite{libovicky2016cuni}.
However, classic automatic evaluation metrics fail to capture the signal in human judgments for the proposed visual story post-editing task.
%We attempt to use automatic evaluation metrics for the proposed visual story automatic post-editing task but fail.
%
We first use the human-edited stories as references, but all the automatic evaluation metrics generate \textit{lower} scores when human judges give a higher rating (Table~\ref{tab:AREL-auto-eval}.)

\begin{comment}



\begin{table}[h]
\center
\scriptsize
\addtolength{\tabcolsep}{-0.12cm} 
\begin{tabular}{L{1.1cm}|rrrr|r}
\textbf{Edited By} & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts} & \textbf{Human} \\ \hline
\textbf{N/A} & 0.93 & 0.59 & 0.92 & 0.97 & \textbf{3.69} \\ \hline
\textbf{LSTM (T)} & 0.26 & 0.24 & 0.42 & 0.76 & \textbf{3.81}
\end{tabular}
\addtolength{\tabcolsep}{0.12cm} 
%\vspace{-.5pc}
\caption{Avg. evaluation scores for AREL. Automatic metrics use human-edited stories as references.}
\label{tab:AREL-auto-eval}
%\vspace{-.5pc}
\end{table}

\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\center
\scriptsize
\addtolength{\tabcolsep}{-0.12cm} 
\begin{tabular}{@{}lrrrrr@{}}
 & \multicolumn{4}{c}{Reference: AREL Stories \textbf{Edited} by Human} & \multicolumn{1}{l}{} \\ \toprule
 & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts} & \textbf{\begin{tabular}[c]{@{}r@{}}Human\\ Rating\end{tabular}} \\ \midrule
\textbf{AREL} & 0.93 & 0.91 & 0.92 & 0.97 & \textbf{3.69} \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}AREL Edited\\ By LSTM(T)\end{tabular}} & 0.21 & 0.46 & 0.40 & 0.76 & \textbf{3.81} \\ \bottomrule
\end{tabular}
\addtolength{\tabcolsep}{0.12cm} 
\caption{Average evaluation scores for AREL stories, using the human-edited stories as references. All the automatic evaluation metrics generate lower scores when human judges give a higher rating.}
\label{tab:AREL-auto-eval}
\end{table}


We then switch to use the human-written stories (VIST test set) as references, but again, all the automatic evaluation metrics generate \textit{lower} scores even when the editing was done by human (Table~\ref{tab:GLAC-auto-eval}.)

\begin{comment}



\begin{table}[h]
\center
\scriptsize
%\footnotesize
\begin{tabular}{l|rrrr}
\textbf{Edited By} & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts} \\ \hline
\textbf{N/A} & \color{red}0.03 & \color{red}0.30 & \color{red}0.26 & 0.66 \\ \hline
\textbf{Human} & \color{red}0.02 & \color{red}0.28 & \color{red}0.24 & 0.65
\end{tabular}
%\vspace{-.5pc}
\caption{Avg. evaluation scores on GLAC stories, using human-written stories as references.}
\label{tab:GLAC-auto-eval}
%\vspace{-.5pc}
\end{table}

\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\center
\scriptsize
\begin{tabular}{@{}lrrrr@{}}
 & \multicolumn{4}{c}{Reference: Human-\textbf{Written} Stories} \\ \toprule
 & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts} \\ \midrule
\textbf{GLAC} & 0.03 & 0.30 & 0.26 & 0.66 \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}GLAC Edited\\ By Human\end{tabular}} & 0.02 & 0.28 & 0.24 & 0.65 \\ \bottomrule
\end{tabular}
\caption{Average evaluation scores on GLAC stories, using human-written stories as references. All the automatic evaluation metrics generate lower scores even when the editing was done by human.}
\label{tab:GLAC-auto-eval}
\end{table}

% \ding{172}
% reference: https://tex.stackexchange.com/questions/199026/how-can-i-draw-circled-integers-with-the-same-size-by-tikz
\begin{table}[t]
\centering
\scriptsize
%\footnotesize
\addtolength{\tabcolsep}{-0.13cm} 
\begin{tabular}{llrrrr}
 & & \multicolumn{4}{c}{Spearman rank-order correlation $\rho$} \\
\toprule \hline
  & \textbf{Data Includes}  & \textbf{BLEU4} & \textbf{METEOR} & \textbf{ROUGE} & \textbf{Skip-Thoughts}\\ \hline
\ding{172} & AREL       & .110   & .099  & .063  & .062           \\
\ding{173} &  LSTM-Edited AREL & .106   & .109  & .067 & .205         \\
\ding{174} & \ding{172}+\ding{173}                     & .095   & .092  & .059    & .116              \\ \hline
\ding{175} & GLAC   & .222   & .203  & .140    &  .151             \\
\ding{176} &  LSTM-Edited GLAC                & .163   & .176  & .138    &    .087           \\
\ding{177} & \ding{175}+\ding{176}                     & .196   & .194  & .148    & .116              \\ \hline
\ding{178} & \ding{172}+\ding{175}                     & .091   & .086  & .059    & .088              \\
\ding{179} & \ding{173}+\ding{176}                     & .089   & .103  & .067    & .101              \\
\ding{180} & \ding{172}+\ding{173}+\ding{175}+\ding{176} & .090   & .096  & .069 & .094             \\ \hline \bottomrule
\end{tabular}
\addtolength{\tabcolsep}{0.13cm} 
\caption{Spearman rank-order correlation $\rho$ between the automatic evaluation scores (sum of all six aspects) and human judgment. 
%When comparing among stories generated by the same visual storytelling model (\ding{175},) BLEU4 and METEOR could still be useful because $\rho$ are similar to that reported by Huang {\em et al.}~\shortcite{huang2016visual}.
%However, 
When comparing
among machine-edited stories (\ding{173} and \ding{176}),
among pre- and post-edited stories (\ding{174} and \ding{177}),
or among any combinations of them (\ding{178}, \ding{179} and \ding{180}),
all metrics result in weak correlations with human judgments.
}
\label{tab:auto-human-cor}
\end{table}

%\kenneth{new text here, need proofread}
Table~\ref{tab:auto-human-cor} further shows the Spearman rank-order correlation $\rho$ between the automatic evaluation scores (sum of all six aspects) and human judgment calculated using different data combination.
In row~\ding{175} of Table~\ref{tab:auto-human-cor}, the reported correlation $\rho$ of METEOR is consistent with the findings in Huang {\em et al.}~\shortcite{huang2016visual}, which suggests that METEOR could be useful when comparing among stories generated by the same visual storytelling model.
%When comparing among stories generated by the same visual storytelling model ({\em e.g.,} row~\ding{175} of Table~\ref{tab:auto-human-cor},) METEOR could still be useful because the correlation $\rho$ are similar to that reported by Huang {\em et al.}~\shortcite{huang2016visual}.
However, when comparing
among machine-edited stories (row \ding{173} and \ding{176}),
among pre- and post-edited stories (row \ding{174} and \ding{177}),
or among any combinations of them (row \ding{178}, \ding{179} and \ding{180}),
all metrics result in weak correlations with human judgments.
%
%the average automatic evaluation scores \textit{decreased} even when the edits were created by humans (Table~\ref{tab:GLAC-auto-eval}.)
These results strongly suggest the need of a new automatic evaluation metric for visual story post-editing task.
%\kenneth{TODO CY/Ed: fill Table~\ref{tab:GLAC-auto-eval}}
Some new metrics have recently been introduced using linguistic~\cite{roemmele2018linguistic} or story features~\cite{purdy2018predicting} to evaluate story automatically.
More research is needed to examine whether these metrics are useful for story post-editing tasks too.





%----------- end of doc ----------------

\begin{comment}


hsu{Some developed system support automated assistance for creative writing, user can freely edit on the stories that automatically generated from RNN Language model based on current stories~\cite{roemmele2018automated}.}
\hsu{Melissa propose linguistic features which is helpful for creative writing~\cite{roemmele2018linguistic}.

Christopher propose story features correlated to human judgments, and provide an algorithm to automatically evaluate the story qualities~\cite{purdy2018predicting}}


\paragraph{Degree of editing did not indicate quality.}
Previous work has shown that APE can be reduced to the Quality Estimation (QE) task because of their similarity in sharing the same inputs but different outputs~\cite{martins2017pushing}. 
QE aims to predict the quality of a machine-translated sentence, in word or sentence level.
APE produced post-edited sentences, which can be viewed as performing three operations for each word: \textit{keep}, \textit{insert}, and \textit{delete}.
QE produced binary labels for each word, indicating if the word requires post-editing.
In this case, positive QE labels are mapped to the \textit{insert} and \textit{delete} operations. Negative QE labels are mapped to the \textit{keep} operation.
Combining both APE and QE into an ensemble model has been demonstrated to have the potential to improve the performance for both tasks~\cite{hokamp2017ensembling}.





We did not present the results of automatic evaluation because 






1. Generalizability (since we only use 2 models)
1-1: Can we generalize to ALL VIST model
1-2: Can we generalize to ALL story generation model

2. We didn't consider the case where users abondon the generated text and write a new one. 
just don't want to edit it, which could also be interesting. Cite Yash/Jeff's paper on ASR editing.


\paragraph{Editing distances can not}
%\input{edit-as-eval}
Creative Help \cite{roemmele2015creative} helps writers by generating the next sentence of a story according to the previous content. 
\citeauthor{roemmele2015creative} evaluated their system by calculating the edit distance \cite{levenshtein1966binary} between the generated sentence and the final result left in the story.
They indicated a good model should result in a low edit distance or, let's say, a few modification. 
We examine this property by checking whether the edit distance of the original story and the human-edited story is negative correlated to the human judge's scores of the original story. The results listed in Table~\ref{tab:edit-auto-correlation} suggests that there is no correlation between the edit distance and the human judge's scores. 

\begin{table}[h]
    \centering
    \scriptsize
    \addtolength{\tabcolsep}{-0.155cm} 
    \begin{tabular}{l|rrrrrr|r}
    \hline
        \textbf{Team} & \textbf{Focused} & \textbf{Coherent} & \textbf{Share} & \textbf{Human} & \textbf{Grounded} & \textbf{Detailed} & \textbf{Average} \\ \hline
        \textbf{AREL} &  0.048 & -0.004 & -0.123 & -0.050 & 0.018 & -0.141 & -0.058 \\
        \textbf{GLAC} & -0.120 & -0.097 &  0.018 & -0.011 & 0.030 & 0.018 & -0.031 \\ \hline 
    \end{tabular}
    \addtolength{\tabcolsep}{0.155cm} 
    \caption{Correlation coefficient between human judge's scores and normalized editing distance.}
    \label{tab:edit-auto-correlation}
\end{table}



the human-edited stories had a lower average automatic evaluation scores than machine-generated stories, as shown in Table~\ref{tab:GLAC-auto-eval}.
All of these results strongly suggest that a new automatic evaluation metrics is needed in order to quickly measure the progress.
\end{comment}

==> ACL_2019_0604(LaTex)/edit-as-eval.tex <==
Compute the correlation coefficient between human judge's scores (1 to 5) and normalized editing distance (0 to 1)



\paragraph{Aggregation Level}
Report a number

\paragraph{Correlation to Each Story Attribute}
Show six (6) numbers




==> ACL_2019_0604(LaTex)/intro.tex <==


Professional writers emphasize the importance of \textit{editing}. Stephen King once put it this way: ``to write is human, to \textit{edit} is divine.''~\cite{king2000writing} Mark Twain had another quote: ``Writing is easy. All you have to do is cross out the wrong words.''~\cite{twain1876adventures}
Given that professionals revise and rewrite their drafts intensively, machines that generate stories may also benefit from a good editor.
%It is hard to argue that, if professional writers need to revise, rewrite, and edit their drafts intensively, machines that generate stories do not need some help from a good editor.  
Per the evaluation of the first Visual Storytelling Challenge~\cite{mitchell2018proceedings}, the ability of an algorithm to tell a sound story is still far from that of a human. Users will inevitably need to edit generated stories before putting them to real uses, such as sharing on social media.
% argument 3: creative work is way more diverse so (1) hard to model, or (2) hard to collect enough data for general purpose (cite IUI paper) -> don't make this argument. We don't have data to support it.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{fig/vist-ape-example.png}
    %\vspace{-1.7pc}
    \caption{A machine-generated visual story (a) (by GLAC), its human-edited (b) and machine-edited (c) (by LSTM) version.}
    \label{fig:vist-ape-example}
    %\vspace{-1.5pc}
\end{figure}

% The story is generated by GLAC and machined-edited by LSTM.

We introduce the first dataset for \textbf{human edits of machine-generated visual stories}, \dataset, and explore how these collected edits may be used for the task of \textit{visual story post-editing} (see Figure~\ref{fig:vist-ape-example}).
The original visual storytelling (VIST) task, as introduced by Huang {\em et al.}~\shortcite{huang2016visual}, takes a sequence of five photos as input and generates a short story describing the photo sequence.
Huang {\em et al.} also released the VIST dataset, containing 20,211 photo sequences, aligned to human-written stories.
On the other hand, the automatic post-editing task revises the story generated from visual storytelling models, given both a machine-generated story and a photo sequence. 
Automatic post-editing treats the VIST system as a black box that is fixed and not modifiable.
Its goal is to correct systematic errors of the VIST system and leverage the user edit data to improve story quality.

In this paper, we \textit{(i)} collect human edits for machine-generated stories from two different state-of-the-art models, \textit{(ii)} analyze what people edited, and \textit{(iii)} advance the task of visual story post-editing.
In addition, we establish baselines for the task, and discuss the weak correlation between automatic evaluation scores and human ratings, motivating the need for new metrics.








%--------------- end of document -----------

\begin{comment}

examine whether edit level indicates the quality of a pre-edited story and establish several baselines for the post-editing task.




%what is VIST
We introduce the first dataset for \textbf{human edits on machine-generated visual stories}, \dataset, and explore how these collected edits may be used for the task of \textit{visual story post-editing.}
The original visual storytelling (VIST) task, as introduced by Huang {\em et al.}~\cite{huang2016visual}, takes a sequence of five photos as input, and generates a short story describing the photo sequence.
The automatic post-editing task, on the other hand, revises the story generated from visual storytelling models, given both machine-generated story and photo sequence.
It treats the VIST system as a black box that is fixed and not modifiable.
The goal of automatic visual story post-editing is to correct systematic errors of VIST system, and leverage the inevitable user edits data to improve the story quality.
In this paper, we 
\textit{(i)} collect human edits for machine-generated stories from two different state-of-the-art models,
\textit{(ii)} analyze what did people edit, and
\textit{(iii)} advance the task of visual story automatic post-editing.
We additionally examine whether the level of edit indicates the quality of pre-edited story, and establish several baselines for the post-editing task. 

Professional writers cannot emphasize enough the importance of \textit{editing}.
Stephen King once put it, ``..., to write is human, to \textit{edit} is divine.''~\cite{king2000writing}
Mark Twain had another quote: ``Writing is easy. All you have to do is cross out the wrong words.''~\cite{twain1876adventures}
It is hard to argue that, if professional writers need to revise, rewrite, and edit their drafts intensively, machines that generate stories do not need some help from a good editor. 
Per the evaluation result of the first Visual Storytelling Challenge~\cite{mitchell2018proceedings}, algorithms' abilities of telling a sound story are still far away from humans.
Users will inevitably need to edit the generated stories before putting them to real uses, {\em e.g.}, sharing on social media.

propose an automatic evaluation metric which is best
correlated with human judgments, and establish several strong baselines for the visual storytelling task.





display these machine-generated stories, aligned with the photo sequences, and had human participants to edit the text, imagining they were going to share it with friends.


and you would like using this story to share your experience with your friends:



first obtain stories generated by two state-of-the-art visual storytelling models, and then display these stories, aligned with the photo sequences, to crowd workers.
We instruct crowd workers 



Among many works that developed using VIST data, we take two state-of-the-art visual storytelling models, AREL (Adversarial REward Learning)~\cite{acl2018wang} and GLAC (Global-Local Attention Cascading)~\cite{kim2018glac} 
 

We ran two visual storytelling models released by Wang {\em et al.}~\cite{acl2018wang} on the test set of VIST to obtain machine-generated visual stories.
Wang's approach was one of the state-of-the-art methods that participated in the first Visual Storytelling Challenge~\cite{mitchell2018proceedings} and also the earliest implementation that was made available online.
\textbf{AREL (Adversarial REward Learning)}~\cite{acl2018wang}: highest METEOR score (0.3179) on public test set.
\textbf{GLAC (Global-Local Attention Cascading)}~\cite{kim2018glac}: highest human evaluation scores (20.295)


%what is VIST APE



the quality of machine-generated stories are still way worse than human-




2nd Draft = 1st Draft – 10\%. Good luck.



In this paper, we introduce a new task, \textit{visual story post-editing}, which takes a visual story generated by an automated system and edit the story text. 



% 1. Why VIST is important? Who can get helped by this?



% 2. Big *BUT* -- why VIST is not good enough now? What's wrong with it?


% 3. What is our solution?


% 4. 1 or 2 sentence to tease our result



Huang {\em et al.} introduced the first dataset VIST for sequential vision-to-language and use automatic evaluation metric for judgment~\cite{huang2016visual}. 


Jing Wang. do automatic generation of paragraph from photo sequence in VIST.  
Kim. use ....
Gonzalez-Rico use ...
Wang. introduce a novel adversarial reward learning algorithm to generate more human-like stories. 

For the prior work, we implemented Adversarial Reward Learning (AREL, which is composed of Baseline and Reward Model) for Visual Storytelling, then evaluate on VIST Dataset. AREL source code is open on Github.

Some text story,

To evaluate the editing distance between AI-editing and Human-editing, we use ... method from Gomaa. survey of text similarity approaches. Machine translation system is also an useful automatic methods for correcting text errors.

Our main idea is that AI-support creative story. Automatic Post-Editing is one of the method. Our goal is that user input 5 individual photos, then we can generated different style of stories which is more reasonable. 

\subsection{Why Post-Editing Matters to Stories?}

``Mostly when I think of pacing, I go back to Elmore Leonard, who explained it so perfectly by saying he just left out the boring parts. This suggests cutting to speed the pace, and that’s what most of us end up having to do (kill your darlings, kill your darlings, even when it breaks your egocentric little scribbler’s heart, kill your darlings)…I got a scribbled comment that changed the way I rewrote my fiction once and forever. Jotted below the machine-generated signature of the editor was this mot: `Not bad, but PUFFY. You need to revise for length. Formula: 2nd Draft = 1st Draft – 10\%. Good luck.' '' — Stephen King, On Writing, 2000~\cite{king2000writing}



\subsection{What?}

\subsection{How?}

\end{comment}

==> ACL_2019_0604(LaTex)/related_work.tex <==



The visual story post-editing task is related to {\em (i)} automatic post-editing and {\em (ii)} stylized visual captioning. \textbf{Automatic post-editing (APE)} revises the text generated typically from a machine translation (MT) system, given both the source sentences and translated sentences. Like the proposed VIST post-editing task, APE aims to correct the systematic errors of MT, reducing translator workloads and increasing productivity~\cite{astudillo2018proceedings}. 
Recently, neural models have been applied to APE in a sentence-to-sentence manner~\cite{libovicky2016cuni,junczys2016log}, differing from previous phrase-based models that translate and reorder phrase segments for each sentence, such as~\cite{simard2007statistical,bechara2011statistical}. More sophisticated sequence-to-sequence models with the attention mechanism were also introduced~\cite{junczys2017exploration,libovicky2017attention}. While this line of work is relevant and encouraging, it has not explored much in a creative writing context.
It is noteworthy that Roemmele {\em et al.} previously developed an online system, Creative Help, for collecting human edits for computer-generated narrative text~\cite{roemmele2018automated}.
The collected data could be useful for story APE tasks.

%, with only a few exceptions using images associated with source text to improve translation quality~\cite{specia2016shared}. 
Visual story post-editing could also be considered relevant to \textbf{style transfer on image captions}. Both tasks take images and source text ({\em i.e.}, machine-generated stories or descriptive captions) as inputs and generate modified text ({\em i.e.}, post-edited stories or stylized captions). End-to-end neural models have been applied to the transfer styles of image captions. For example, \textit{StyleNet}, an encoder-decoder-based model trained on paired images and factual captions together with an unlabeled stylized text corpus, can transfer descriptive image captions to creative captions, {\em e.g.,} humorous or romantic~\cite{gan2017styleNet}. Its advanced version with an attention mechanism, \textit{SemStyle}, was also introduced~\cite{mathews2018semstyle}.
In this paper, we adopt the APE approach to treat pre- and post-edited stories as parallel data instead of the style transfer approach that omits this parallel relationship during model training.


%used an recurrent neural network model to generate suggestions for creative writing, and users can freely edit on the machine-generated


%Some developed system support automated assistance for creative writing, user can freely edit on the stories that automatically generated from RNN Language model based on current stories~\cite{roemmele2018automated}.




%\kenneth{TODO Edward: Add new citations in the following, describing them why they're relevant.}

%\hsu{Some developed system support automated assistance for creative writing, user can freely edit on the stories that automatically generated from RNN Language model based on current stories~\cite{roemmele2018automated}.}
%\hsu{Melissa propose linguistic features which is helpful for creative writing~\cite{roemmele2018linguistic}. Christopher propose story features correlated to human judgments, and provide an algorithm to automatically evaluate the story qualities~\cite{purdy2018predicting}}




%\paragraph{Stylized Visual Captioning and Storytelling}




%========== end of doc ================

\begin{comment}


In this paper, we took the route closer to APE because pre- and post-edited stories are, by its nature, a form of parallel data, whereas neither StyleNet nor SemStyle used labeled parallel data for training.




The visual story automatic post-editing task is related to {\em (i)} automatic post-editing and {\em (ii)} stylized visual captioning.
\textbf{Automatic post-editing (APE)} revises the text generated from, usually, a machine translation (MT) system, given both the source sentences and translated sentences. 
%The MT system is treated as a black box that is fixed and not modifiable.
Similar to the proposed VIST post-editing task, APE aims to correct systematic errors of MT, reducing translators' workload and increasing productivity~\cite{astudillo2018proceedings}.
Recently, neural models have been applied for APE in a sentence-to-sentence manner~\cite{libovicky2016cuni,junczys2016log}, differing from previous phrase-based models that translate and reorder phrase segments for each sentence, such as~\cite{simard2007statistical,bechara2011statistical}. 
More sophisticated sequence-to-sequence models with the attention mechanism were also introduced~\cite{junczys2017exploration,libovicky2017attention}.
While this line of work is relevant and encouraging, it has not explored much under a multimodal context, with only a few exceptions using images associated with source text to improve translation quality~\cite{specia2016shared}.
Visual story post-editing could also be viewed relevant to \textbf{style transfer on image captions}. 
Both tasks takes images and source text ({\em i.e.}, machine-generated story, or descriptive caption) in order to generate modified text ({\em i.e.}, post-edited story, or stylized captions). 
End-to-end neural approaches have been applied to transfer styles of image captions. 
For example, \textit{StyleNet}, an encoder-decoder-based model trained on paired images and factual-captions, together with unlabeled stylized text corpus, can transfer descriptive image captions to attractive captions, {\em e.g.,} humorous or romantic~\cite{gan2017styleNet}.
Its advanced version with the attention mechanism, \textit{SemStyle}, was also introduced~\cite{mathews2018semstyle}.

Beyond captioning, visual storytelling focuses on creating engaging narratives by making sense of a series of images~\cite{huang2016visual}. One recent work developed a model to generate coherent stories from photo streams by using adversarial training, which involved a generator and several discriminators~\cite{wang2018show,acl2018wang}.

Similar to Generative Adversarial Nets~\cite{goodfellow2014generative}, the generator tries to create human-indistinguishable stories while the discriminators learn to determine if the created stories are relevant to the input images and resemble the human writing style. The adversarial training strategy applies deep reinforcement learning, where the generator is improved by using the discriminator. The generator is analogous to an agent's policy function, which maps states to actions. Each input image represents the current state, and each output sentence represents the best action. The discriminator is analogous to an environment, which is a function that provides the ground-truth reward for correcting the estimated reward computed by the generator. The training process iterates until the discriminator is unable to determine whether a story is created by a human or the generator. 

In the context of visual storytelling, the generator is a hierarchical model that concatenates multiple encoder-decoder networks in parallel, which has been adopted for generating a paragraph from every image \cite{krause2016para}. The hierarchical structure simplifies the visual storytelling challenge to a one-to-one mapping between photo streams and sentences. The discriminators are CNN-based (or RNN-based) classifiers (or regressors), which provide scores to indicate if the generated story resembles human-level style.







which differs from template matching~\cite{kulkarni2013babytalk} and image-text aligning~\cite{farhadi2010every,zhu2015aligning,karpathy2014deep}.






APE in a sentence-to-sentence manner~\cite{libovicky2016cuni,junczys2016log}, differing from previous phrase-based models that translate and reorder phrase segments for each sentence, such as~\cite{simard2007statistical,bechara2011statistical}. 



%This setup is similar to \textbf{style transfer on image captions}, 




One approach is to use computer vision and deep learning to generate attractive ``stylized'' captions directly for images or videos. 

This approach is end-to-end, which differs from template matching~\cite{kulkarni2013babytalk} and image-text aligning~\cite{farhadi2010every,zhu2015aligning,karpathy2014deep}.

This approach is also different from generating ``factual'' captions that describe the actual situation in images, such as~\cite{vinyals2015show,venugopalan2015sequence,xu2015show,mnih2014recurrent}.

One can consider captioning as a special type of machine translation problem that converts source images (instead of sentences in a source language) into sentences in a target language. Therefore, the encoder-decoder framework that integrates two deep neural networks, which has been adopted in neural machine translation~\cite{cho2014learning,sutskever2014sequence,bahdanau2014neural}, can be naturally applied for this task.

One example is \textit{StyleNet}, an encoder-decoder based model for learning romantic and humorous captions~\cite{gan2017styleNet}. \textit{StyleNet} consists of a convolutional neural network (CNN) and many recurrent neural networks (RNN) that act as an encoder and decoders respectively. The CNN encodes images into a fixed-length vector, which represents a data point in a high dimensional space. The RNNs decode the vector into captions with various lengths and styles. The training data of \textit{StyleNet} includes paired images and factual-captions, together with unlabeled romantic-style and humorous-style text corpus. The decoders are trained by using multi-task learning (MTL), where the training phase alternates among several tasks~\cite{luong2015multi}. Training the main task (e.g., language-to-language machine translation) with several additional tasks (e.g., image captioning or unsupervised learning) jointly can increase the performance of the main task~\cite{luong2015multi}. During training, both the parameters in the decoders and encoders can be shared, depending on the type of the main task. MTL works in parallel, which differs from the sequential approach that the model is first pretrained and then finetuned, such as~\cite{dai2015semi}.

Another example of generating stylized captions is the \textit{SemStyle} system~\cite{mathews2018semstyle}, which also adopted the encoder-decoder network. Both the encoder and decoder were trained separately on image caption datasets and a large text corpus respectively. The encoder mapped images to semantics terms, and the decoder converted semantics terms into sentences. Different from \textit{StyleNet} that took the latest output of the encoder as input for the decoder, \textit{SemStyle} added the attention mechanism. This idea is analogous to the attention mechanism in machine translation, which allows the decoder to access multiple outputs from the encoder, instead of using only the output from the final layer of the encoder~\cite{bahdanau2014neural,luong2015effective}. Attention mitigates the issue of information loss due to the intermediate step that encodes the input into a fixed-length vector in the typical encoder-decoder model.

Beyond captioning, visual storytelling focuses on creating engaging narratives by making sense of a series of images~\cite{huang2016visual}. One recent work developed a model to generate coherent stories from photo streams by using adversarial training, which involved a generator and several discriminators~\cite{wang2018show,acl2018wang}. Similar to Generative Adversarial Nets~\cite{goodfellow2014generative}, the generator tries to create human-indistinguishable stories while the discriminators learn to determine if the created stories are relevant to the input images and resemble the human writing style. The adversarial training strategy applies deep reinforcement learning, where the generator is improved by using the discriminator. The generator is analogous to an agent's policy function, which maps states to actions. Each input image represents the current state, and each output sentence represents the best action. The discriminator is analogous to an environment, which is a function that provides the ground-truth reward for correcting the estimated reward computed by the generator. The training process iterates until the discriminator is unable to determine whether a story is created by a human or the generator. In the context of visual storytelling, the generator is a hierarchical model that concatenates multiple encoder-decoder networks in parallel, which has been adopted for generating a paragraph from every image \cite{krause2016para}. The hierarchical structure simplifies the visual storytelling challenge to a one-to-one mapping between photo streams and sentences. The discriminators are CNN-based (or RNN-based) classifiers (or regressors), which provide scores to indicate if the generated story resembles human-level style.



For example, Libovicky {\em et al.} developed an APE system with many encoders and a decoder, where the input of the encoders are pairs of original sentences and machine-translated sentences and the output of the decoder are post-edited sentences~\cite{libovicky2016cuni}.
Junczys-Dowmunt and Grundkiewicz



%To prevent the model from paraphrasing the original sentences instead of editing them, the post-edited sentences are represented as a sequence of edit operations: \textit{keep}, \textit{delete}, and \textit{insert}.
Another system, proposed by Junczys-Dowmunt and Grundkiewicz, adopted an ensemble-based approach to combined multiple deep neural networks with a log-linear model~\cite{junczys2016log}.
This approach enabled each component in the ensemble to take different inputs, including the post-edited and machine-translated sentences.

While this is an encouraging first
step in connecting vision and language, it is far from
the capabilities needed by intelligent agents for naturalistic interactions





\subsection{Stylized Visual Captioning and Storytelling}

One approach is to use computer vision and deep learning to generate attractive ``stylized'' captions directly for images or videos. This approach is end-to-end, which differs from template matching~\cite{kulkarni2013babytalk} and image-text aligning~\cite{farhadi2010every,zhu2015aligning,karpathy2014deep}. This approach is also different from generating ``factual'' captions that describe the actual situation in images, such as~\cite{vinyals2015show,venugopalan2015sequence,xu2015show,mnih2014recurrent}. One can consider captioning as a special type of machine translation problem that converts source images (instead of sentences in a source language) into sentences in a target language. Therefore, the encoder-decoder framework that integrates two deep neural networks, which has been adopted in neural machine translation~\cite{cho2014learning,sutskever2014sequence,bahdanau2014neural}, can be naturally applied for this task.

One example is \textit{StyleNet}, an encoder-decoder based model for learning romantic and humorous captions~\cite{gan2017styleNet}. \textit{StyleNet} consists of a convolutional neural network (CNN) and many recurrent neural networks (RNN) that act as an encoder and decoders respectively. The CNN encodes images into a fixed-length vector, which represents a data point in a high dimensional space. The RNNs decode the vector into captions with various lengths and styles. The training data of \textit{StyleNet} includes paired images and factual-captions, together with unlabeled romantic-style and humorous-style text corpus. The decoders are trained by using multi-task learning (MTL), where the training phase alternates among several tasks~\cite{luong2015multi}. Training the main task (e.g., language-to-language machine translation) with several additional tasks (e.g., image captioning or unsupervised learning) jointly can increase the performance of the main task~\cite{luong2015multi}. During training, both the parameters in the decoders and encoders can be shared, depending on the type of the main task. MTL works in parallel, which differs from the sequential approach that the model is first pretrained and then finetuned, such as~\cite{dai2015semi}.

Another example of generating stylized captions is the \textit{SemStyle} system~\cite{mathews2018semstyle}, which also adopted the encoder-decoder network. Both the encoder and decoder were trained separately on image caption datasets and a large text corpus respectively. The encoder mapped images to semantics terms, and the decoder converted semantics terms into sentences. Different from \textit{StyleNet} that took the latest output of the encoder as input for the decoder, \textit{SemStyle} added the attention mechanism. This idea is analogous to the attention mechanism in machine translation, which allows the decoder to access multiple outputs from the encoder, instead of using only the output from the final layer of the encoder~\cite{bahdanau2014neural,luong2015effective}. Attention mitigates the issue of information loss due to the intermediate step that encodes the input into a fixed-length vector in the typical encoder-decoder model.

Beyond captioning, visual storytelling focuses on creating engaging narratives by making sense of a series of images~\cite{huang2016visual}. One recent work developed a model to generate coherent stories from photo streams by using adversarial training, which involved a generator and several discriminators~\cite{wang2018show,acl2018wang}. Similar to Generative Adversarial Nets~\cite{goodfellow2014generative}, the generator tries to create human-indistinguishable stories while the discriminators learn to determine if the created stories are relevant to the input images and resemble the human writing style. The adversarial training strategy applies deep reinforcement learning, where the generator is improved by using the discriminator. The generator is analogous to an agent's policy function, which maps states to actions. Each input image represents the current state, and each output sentence represents the best action. The discriminator is analogous to an environment, which is a function that provides the ground-truth reward for correcting the estimated reward computed by the generator. The training process iterates until the discriminator is unable to determine whether a story is created by a human or the generator. In the context of visual storytelling, the generator is a hierarchical model that concatenates multiple encoder-decoder networks in parallel, which has been adopted for generating a paragraph from every image \cite{krause2016para}. The hierarchical structure simplifies the visual storytelling challenge to a one-to-one mapping between photo streams and sentences. The discriminators are CNN-based (or RNN-based) classifiers (or regressors), which provide scores to indicate if the generated story resembles human-level style.

\subsection{Neural Automatic Post-Editing}

Another approach is neural automatic post-editing (APE), which uses deep learning to automatically revises the text generated from a machine translation (MT) system, given both the source sentences (or images in our case) and translated sentences. The MT is treated as a black-box system that is fixed and not modifiable. The goal of APE is to correct systematic MT errors, thereby reducing translators' workload and eventually increasing translation productivity~\cite{astudillo2018proceedings}. APE is different from computer-assisted post-editing, which aims to develop interactive systems that suggest modifications based on human guidance, such as~\cite{grangier2018quickedit,peris2017interactive}. Additionally, neural APE is sentence-to-sentence, which differs from previous state-of-the-art phrase-based models that translate and reorder phrase segments for each sentence, such as~\cite{simard2007statistical,bechara2011statistical}. One can also view APE as a multimodal translation problem, where MT generated sentences are translated into post-edited sentences with the source images as additional information~\cite{specia2016shared}.

The encoder-decoder model has been applied to automatic post-editing. For instance, Libovicky et al. developed a system with many encoders and a decoder~\cite{libovicky2016cuni}. The input of the encoders are pairs of original sentences and machine-translated sentences. The output of the decoder are post-edited sentences. To prevent the model from paraphrasing the original sentences instead of editing them, the post-edited sentences are represented as a sequence of edit operations: \textit{keep}, \textit{delete}, and \textit{insert}. Another system, proposed by Junczys-Dowmunt and Grundkiewicz, adopted an ensemble-based approach to combined multiple deep neural networks with a log-linear model~\cite{junczys2016log}. This approach enabled each component in the ensemble to take different inputs, including the post-edited and machine-translated sentences. The system overcame the problem of limited APE training data by generating a large amount of artificial training data with back-translation~\cite{sennrich2015improving}. The idea was to use two phase-based MT systems to translate German to English and then back to German. The original German, the translated English, and the back-translated German are treated as the post-edited, source, and the machine-translated sentences respectively. Model sophisticated sequence-to-sequence learning models with the attention mechanism that extended these two works were later proposed~\cite{junczys2017exploration,libovicky2017attention}.

Previous work has shown that APE can be reduced to the Quality Estimation (QE) task because of their similarity in sharing the same inputs but different outputs~\cite{martins2017pushing}. QE aims to predict the quality of a machine-translated sentence, in word or sentence level. APE produced post-edited sentences, which can be viewed as performing three operations for each word: \textit{keep}, \textit{insert}, and \textit{delete}. QE produced binary labels for each word, indicating if the word requires post-editing. In this case, positive QE labels are mapped to the \textit{insert} and \textit{delete} operations. Negative QE labels are mapped to the \textit{keep} operation. Combining both APE and QE into an ensemble model has been demonstrated to have the potential to improve the performance for both tasks~\cite{hokamp2017ensembling}.


\end{comment}

==> edit-as-eval.tex <==
Compute the correlation coefficient between human judge's scores (1 to 5) and normalized editing distance (0 to 1)



\paragraph{Aggregation Level}
Report a number

\paragraph{Correlation to Each Story Attribute}
Show six (6) numbers



